(Machine) Learning What Policies Value

When a policy prioritizes one person over another, is it because they benefit more, or because they are preferred? This paper develops a method to uncover the values consistent with observed allocation decisions. We use machine learning methods to estimate how much each individual benefits from an intervention, and then reconcile its allocation with (i) the welfare weights assigned to different people; (ii) heterogeneous treatment effects of the intervention; and (iii) weights on different outcomes. We demonstrate this approach by analyzing Mexico's PROGRESA anti-poverty program. The analysis reveals that while the program prioritized certain subgroups -- such as indigenous households -- the fact that those groups benefited more implies that they were in fact assigned a lower welfare weight. The PROGRESA case illustrates how the method makes it possible to audit existing policies, and to design future policies that better align with values.

==> Code/figs/simulations.tex <==
\begin{figure}
\begin{tabular}{cc}
\multicolumn{2}{c}{\textbf{An allocation rule that prioritizes the poor (low $x_i$)...}}\\
\multicolumn{2}{c}{\includegraphics[width=5cm]{./Code/figs/simulations/1D_IMU_Z}}\\
\multicolumn{1}{l}{\textbf{Could result from}} & \\
Higher welfare weight on the poor & if treatment effects are constant\\
\includegraphics[width=5cm]{./Code/figs/simulations/1D_EMU_MU} & \includegraphics[width=5cm]{./Code/figs/simulations/1D_EMU_DeltaG}\\
Equal welfare weights on households & if treatment effects are higher for the poor\\
\includegraphics[width=5cm]{./Code/figs/simulations/1D_DMU_MU} & \includegraphics[width=5cm]{./Code/figs/simulations/1D_DMU_DeltaG}\\
Higher welfare weight on the rich & if treatment effects are much higher for the poor\\
\includegraphics[width=5cm]{./Code/figs/simulations/1D_IMU_MU} & \includegraphics[width=5cm]{./Code/figs/simulations/1D_IMU_DeltaG}\\
\end{tabular}
\caption{Intuitive Example\label{fig:Intuitive-Example}}
\end{figure}
\vfill{}

==> Code/tables/preferences_vs_survey_deprecated.tex <==

\begin{table}
\centering \caption{Assessing Decision Rules\label{tab:Allocation-Rule-Actual-Survey}}
\global\long\def\arraystretch{1.2}%
 \begin{threeparttable} 
\begin{centering}
{\footnotesize{}}%
\begin{tabular}{l>{\raggedleft}p{2.7cm}>{\raggedleft}p{0.4cm}>{\raggedleft}p{2.7cm}>{\raggedleft}p{2.7cm}}
 & \multicolumn{3}{c}{{\footnotesize{}Household Poverty Score}} & \tabularnewline
 &  &  &  & \tabularnewline
 & \multicolumn{1}{>{\raggedleft}p{3cm}}{{\footnotesize{}Without Accounting for Heterogeneous TE variation}} &  & \multicolumn{2}{c}{{\footnotesize{}Accounting for variation in TE}}\tabularnewline
 & {\scriptsize{}1999 Ranking} &  & {\scriptsize{}1999 Ranking} & {\scriptsize{}2003 Ranking}\tabularnewline
 &  &  &  & \tabularnewline
 & \multicolumn{1}{>{\centering}p{2.4cm}}{\textbf{\footnotesize{}Log Welfare Weights $log_{1.01}(\boldsymbol{\omega})$}}  & \multicolumn{3}{>{\centering}p{2.7cm}}{\textbf{\footnotesize{}Log Welfare Weights $log_{1.01}(\boldsymbol{\omega})$}}\tabularnewline
{\footnotesize{}log(Income)} & {\footnotesize{}-21.393 (2.401)} &  & {\footnotesize{}-11.194 (4.002)} & {\footnotesize{}-2.370 (1.469)}\tabularnewline
{\footnotesize{}Household Size} & {\footnotesize{}12.961 (0.943)} &  & {\footnotesize{}4.970 (1.676)} & {\footnotesize{}2.706 (1.252)}\tabularnewline
{\footnotesize{}Head Age} & {\footnotesize{}-2.267 (0.244)} &  & {\footnotesize{}-1.176 (0.578)} & {\footnotesize{}-0.232 (0.157)}\tabularnewline
{\footnotesize{}Education} & {\footnotesize{}-4.119 (0.884)} &  & {\footnotesize{}-3.181 (1.219)} & {\footnotesize{}-1.945 (0.969)}\tabularnewline
{\footnotesize{}Indigenous} & {\footnotesize{}44.080 (5.996)} &  & {\footnotesize{}-9.762 (3.625)} & {\footnotesize{}2.839 (3.589)}\tabularnewline
 &  &  &  & \tabularnewline
 &  &  \multicolumn{3}{>{\centering}p{2.7cm}}{\textbf{\footnotesize{}Impact Weights $\mathbf{\lambda}$}}\tabularnewline
 &  &  & \multicolumn{2}{c}{}\tabularnewline
{\footnotesize{}Sickness (per child sick day)} &  & \textbf{\footnotesize{}$\lambda_{1}$} & {\footnotesize{}0.074 (0.058)} & {\footnotesize{}0.151 (0.105)}\tabularnewline
{\footnotesize{}Missed Schooling (per day)} &  & \textbf{\footnotesize{}$\lambda_{2}$} & {\footnotesize{}-0.049 (0.167)} & {\footnotesize{}0.005 (0.192)}\tabularnewline
 &  &  & \multicolumn{2}{c}{}\tabularnewline
{\footnotesize{}Value Regardless of Impact} &  & {\footnotesize{}$C$} & {\footnotesize{}0.495 (2.176)} & {\footnotesize{}1.620 (4.525)}\tabularnewline
 &  &  &  & \tabularnewline
 &  & {\footnotesize{}$\sigma$} & {\footnotesize{}0.138 (0.131)} & {\footnotesize{}0.241 (0.158)}\tabularnewline
 &  &  &  & \tabularnewline
{\footnotesize{}N} & {\footnotesize{}6642} &  & {\footnotesize{}6642} & {\footnotesize{}6642}\tabularnewline
\end{tabular}\begin{tablenotes}[normal,flushleft] 
{\footnotesize{}\item }\emph{\footnotesize{}Notes}{\footnotesize{}:
Left column computed using our method, using heterogeneous treatment
effects estimated with causal forest (see Figure~\ref{fig:Distribution-of-Estimated-CF}).
Right column reports revealed preference estimates from an online
survey of Mexican residents. (N.B. that survey estimates use same value for $C$ impact weight as that inferred from our method.) In left column, standard errors are computed
using a two-step bootstrap procedure that accounts for uncertainty
in both treatment effects and preference parameters. Observations
are drawn with replacement before estimation of the treatment effects
and the welfare and impact weights. Treatment effects are then estimated
from these bootstrapped samples, and welfare and impact weights estimated
from these bootstrapped treatment effect estimates; the standard errors
reported are the standard deviation across bootstrapped welfare and
impact weight estimates. Some respondents in survey did not respond
to all questions.d \end{tablenotes} }{\footnotesize\par}
\par\end{centering}
\end{threeparttable} 
\end{table}


